MEANTIME: Mixture of Attention Mechanisms with Multi-temporal Embeddings for Sequential Recommendation

Recently, self-attention based models have achieved state-of-the-art performance in sequential recommendation task. Following the custom from language processing, most of these models rely on a simple positional embedding to exploit the sequential nature of the user's history. However, there are some limitations regarding the current approaches. First, sequential recommendation is different from language processing in that timestamp information is available. Previous models have not made good use of it to extract additional contextual information. Second, using a simple embedding scheme can lead to information bottleneck since the same embedding has to represent all possible contextual biases. Third, since previous models use the same positional embedding in each attention head, they can wastefully learn overlapping patterns. To address these limitations, we propose MEANTIME (MixturE of AtteNTIon mechanisms with Multi-temporal Embeddings) which employs multiple types of temporal embeddings designed to capture various patterns from the user's behavior sequence, and an attention structure that fully leverages such diversity. Experiments on real-world data show that our proposed method outperforms current state-of-the-art sequential recommendation methods, and we provide an extensive ablation study to analyze how the model gains from the diverse positional information.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'nonacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
                Font changes for SIGCHI table captions

Version 1.56    Bug fixes
                Added \flushbottom to two column formats (Philip Quinn)
                The final punctuation for the list of concepts
                is now a period instead of a semicolon (Philip Quinn)
                New command \Description to describe images for visually
                impaired users.

Version 1.57    Change of \baselinestretch now produces an error
                Booktabs is now always loaded
                Added option `balance' to balance last page in two-column mode
                E-mail is no longer split in addresses
                New samples (Stephen Spencer)

Version 1.58    Suppressed spurious warnings.
		New journal:  HEALTH.
		TDSCI is renamed to TDS.

Version 1.59    Now a journal format can be used for conference proceedings
		All samples are now generated from the same .dtx file
		Bug fixes

version 1.60    New option: urlbreakonhyphens (thanks to Peter Kemp)
		Smaller header size for acmsmall

Version 1.61    Bug fixes
                New bibtex types for artifacts

Version 1.62    Documentation update
		New journal: TELO
		Bug fixes

Version 1.63	New journals: TQUANT, FACMP

Version 1.63a   Moved TQUANT to TQC

Version 1.64    Produce error if abstract is entered after maketitle
		(previously abstract was silently dropped)
		Bug fixes for line numbering

Version 1.65   Bug fixes
	       New journal: DGOV
	       DTRAP and HEALTH are now using acmlarge format

Version 1.66   Bug fixes
	       BibTeX change:  location is now a synonym for city (Feras Saad) 
	       ACM reference format is now mandatory for papers over one page.
	       CCS concepts and keywords are now mandatory for
	       papers over two pages.
	       Authors' addresses are mandatory for journal articles.

Version 1.67   Urgent bug fixes:
	       BibTeX style bug fixed (Michael D. Adams)
	       Sigplan special section bugfix

Version 1.68   Bug fixes
               BST now recognizes words `Paper' or 'Article' in
	       eid or articleno

Version 1.69   Bug fixes
	       Compatibility with LaTeX 2020-02-02 release


==> sections/experiments_subsections/attn_map.tex <==
\begin{figure}[ht]
  \centering
  
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L0BPH1.png}
    \caption{\textbf{Pos} Layer 0 Head 1}
  \end{subfigure}
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L0BDH0.png}
    \caption{\textbf{Day} Layer 0 Head 0}
  \end{subfigure}
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L0BCH0.png}
    \caption{\textbf{Const} Layer 0 Head 0}
  \end{subfigure}
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L0BSH0.png}
    \caption{\textbf{Sinusoid} Layer 0 Head 0}
  \end{subfigure}
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L0BEH0.png}
    \caption{\textbf{Exp} Layer 0 Head 0}
  \end{subfigure}
  \begin{subfigure}[ht]{.33\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/attn1/L1BLH0.png}
    \caption{\textbf{Log1p} Layer 1 Head 0}
  \end{subfigure}
  
  %\subfigure{\includegraphics[width=0.5\linewidth]{figures/attn1/L0BDH0.png}}
  %\subfigure{\includegraphics[width=0.5\linewidth]{figures/attn1/L0BDH1.png}}
  \caption{Attention Score Maps (Might need to change the figures to ones with shorter sequences (so that they are more clear))}
  \Description{TODO:Description}
  \label{fig:attnmaps}
\end{figure}


==> sections/experiments_subsections/combinations.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[ht]{.49\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/tesearch.png}
    \caption{MovieLens 1M}
  \end{subfigure}
  \begin{subfigure}[ht]{.49\linewidth}
    \centering\includegraphics[width=.95\linewidth]{figures/tesearch_game.png}
    \caption{Amazon Game}
  \end{subfigure}
  \caption{NDCG@10 Comparison with All Possible Combinations of Positional Embeddings on ML-1M and Game Dataset}
  \Description{TODO:Description}
  \label{fig:tesearch}
\end{figure}

==> sections/experiments_subsections/effect_freq_tau.tex <==
\begin{figure}[ht]
  \centering
  \begin{subfigure}[ht]{.45\linewidth}
    \centering\includegraphics[width=\linewidth]{figures/freq_tau/freq_search.png}
    \caption{Effect of \textit{freq}}
  \end{subfigure}
  \begin{subfigure}[ht]{.45\linewidth}
    \centering\includegraphics[width=\linewidth]{figures/freq_tau/tau_search.png}
    \caption{Effect of $\tau$}
  \end{subfigure}
  \caption{Effect of \textit{freq} and $\tau$ on performance}
  \Description{TODO:Description}
  \label{fig:freq_tau}
\end{figure}

==> sections/experiments_subsections/effect_hsize.tex <==
Here we study the effect of hidden dimension size on each dataset. We experiment with $h \in \{16, 32, 64, 128\}$ while keeping other hyperpameters the same.

\begin{figure}[ht]
  \centering
  
  \begin{subfigure}[ht]{\linewidth}
    \centering\includegraphics[width=\linewidth]{figures/impact_h/n10.png}
    \caption{NDCG@10}
  \end{subfigure}
  \begin{subfigure}[ht]{\linewidth}
    \centering\includegraphics[width=\linewidth]{figures/impact_h/r10.png}
    \caption{Recall@10}
  \end{subfigure}
  
  \caption{Effect of hidden dimension size on NDCG@10 and Recall@10}
  \Description{TODO:Description}
  \label{fig:himpact}
\end{figure}

Figure-\ref{fig:himpact} shows the comparison results. We observe that optimal hidden dimension size differs between datasets. Interestingly, MEANTIME works optimally at $h = 16$ in Amazon Beauty dataset. This is probably because it is the most sparse dataset of the four, which makes it prone to overfitting.

We also observe that without extensive hyperparameter tuning, TiSASRec\cite{TISASRec}, which uses temporal infromation to improve SASRec\cite{SASRec}, sometimes doesn't outperform SASRec. In contrast, MEANTIME, which improves BERT4Rec\cite{BERT4Rec} with temporal information, always outperforms BERT4Rec (and all other baseline models) even without parameter tuning. This seems to prove the superiority of our model. [TOO MUCH BRAGGING?]

==> sections/experiments_subsections/effect_multiblocks.tex <==
Although we let all transformer-based models have the same number of layers and heads in our experiments, MEANTIME has more parameters than SASRec, TiSASRec, and BERT4Rec since it employs 6 self-attention blocks per layer in contrast to 1. This might seem unfair since the performance gain could have come from the larger parameter size, or from the multi-path self-attention. To prove that this is not the case, we also experimented with the adjusted baseline models where they also have 6 self-attention blocks per layer. We call them \textbf{buffed} models. 

\begin{table}[h]
\caption{Performance Comparison with Buffed Baselines.}
\label{tab:buff_results}
\begin{tabular}{@{}lrrrrr@{}}
\toprule
{Metrics} & {SASRec-Buffed}& {TiSASRec-Buffed} & {BERT4Rec-Buffed} & {MEANTIME}      \\ \midrule
{Recall@5}  & {0.5512} & {0.5528} & {0.5916} & {\textbf{0.6154}} \\
{Recall@10}  & {0.6853} & {0.6856} & {0.6987} & {\textbf{0.7268}} \\
{NDCG@5}   & {0.3955} & {0.3962}  & {0.4437} & {\textbf{0.4690}} \\
{NDCG@10}  & {0.4390} & {0.4393}  & {0.4785} & {\textbf{0.5052}} \\ \bottomrule
\end{tabular}
\end{table}

Table-\ref{tab:buff_results} shows the comparison results. All experiments were done with ML-1M dataset, hidden dimension size $h=64$, dropout ratio 0.2 and weight decay 0. The result clearly shows that the strong performance of MEANTIME does not merely come from large parameter size nor multi-path self-attention.

==> sections/experiments_subsections/grad_cam.tex <==
\begin{table}[ht]
\caption{Gradient Comparison for Each Embedding Type}
\label{tab:grad_cam}
\begin{tabular}{@{}lllllll@{}}
\toprule
{Dataset} & {Pos}           & {Day}              & {Const}            & {Sinusoid}         & {Exp}           & {Log1p}         \\ \midrule
{ML1M}    & {4.79\%}        & {5.34\%}           & {1.50\%}           & {\textbf{51.34\%}} & {7.08\%}        & {\underline{29.94\%}} \\
{ML20M}   & {\underline{19.60\%}} & {5.50\%}           & {6.11\%}           & {\textbf{24.51\%}} & {\underline{22.58\%}} & {\underline{21.70\%}} \\
{Beauty}  & {1.03\%}        & {8.39\%}           & {\textbf{57.12\%}} & {9.79\%}           & {0.69\%}        & {\underline{22.98\%}} \\
{Game}    & {\underline{40.39\%}} & {\textbf{49.57\%}} & {1.96\%}           & {1.19\%}           & {1.37\%}        & {5.51\%}  \\ \bottomrule
\end{tabular}
\end{table}

==> sections/method_subsections/absolute_pe.tex <==
Given $s$ and $t$, any absolute position embedding layer should return a matrix of the form $\mathbf{E}^p \in \mathbb{R}^{N \times h}$: where each row $p_i \in \mathbb{R}^h$ is a representation of the $i^{th}$ position in a sequence of length $N$. We devised three ways to generate such a matrix.

\begin{displaymath}
  \mathbf{E}^{day} = \begin{bmatrix}
                      m_{day_1}\\
                      m_{day_2}\\
                      ...\\
                      m_{day_n}\\
                    \end{bmatrix}
  ,\mathbf{E}^{pos} = \begin{bmatrix}
                       pos_1\\
                       pos_2\\
                       ...\\
                       pos_n\\
                     \end{bmatrix}\\
  , 
  \mathbf{E}^{const} = \begin{bmatrix}
                       c\\
                       c\\
                       ...\\
                       c\\
                       \end{bmatrix}   
\end{displaymath}

The first is \textbf{Day}-embedding, where we represent each position by the day of its timestamp $t_i$ (as in \textit{how many days}, not as in \textit{Monday, Tuesday, ...}). More specifically, we keep a learnable embedding matrix $\mathbf{M}^D \in \mathbb{R}^{|D| \times h}$ where $|D|$ is the number of possible days in the span of the dataset. We convert each timestamp into its corresponding day, and then do an embedding lookup operation to get $\mathbf{E}^{day}$. We figured that \textbf{Day} is a reasonable choice for time unit since smaller time units can make the size of the embedding matrix too large, while larger time units can easily miss the delicate differences between each time period.

\textbf{Pos}-embedding is analogous to the learnable positional embeddings used in \cite{BERT, BERT4Rec}, where each $pos_i$ is a learnable vector that represents the $i^{th}$ position, regardless of the input timestamps. \textbf{Const}-embedding is similar to \textbf{Pos}-embedding, except that all position vectors are shared. This removes positional biases so that we can focus only on the relationship between tokens' contents. The constant vector $c$ functions as a bias towards certain contents.

Note that we don't add these positional embeddings to the token embeddings as in \cite{BERT, BERT4Rec}. We just pass them to the related self-attention blocks where we handle these embeddings separately. This prevents mix-ups between content and positional information, which is beneficial as will be shown in later ablation studies.


==> sections/method_subsections/relative_pe.tex <==
Given $s$ and $t$, any relative position embedding layer should return a matrix of the form $\mathbf{E}^r \in \mathbb{R}^{N \times N \times h}$: where each $r_{ij} \in \mathbb{R}^h$ represents the relationship between $i^{th}$ and $j^{th}$ positions. First, we create a matrix of differences between timestamps:
\begin{displaymath}
  \mathbf{D} = \begin{bmatrix}
                    d_{11} & d_{12} & ... & d_{1n}\\
                    d_{21} & d_{22} & ... & d_{2n}\\
                    ... & ... & ... & ...\\
                    d_{n1} & d_{n2} & ... & d_{nn}
                    \end{bmatrix}
\end{displaymath}
where $d_{ij} = \frac{t_i - t_j}{\tau}$ and $\tau$ is an adjustable parameter.

Next, we apply unique encoding functions to create three relative position embeddings:

\begin{displaymath}
\mathbf{E}^{sinusoid} = \begin{bmatrix}
                    \theta_{11} & \theta_{12} & ... & \theta_{1n}\\
                    \theta_{21} & \theta_{22} & ... & \theta_{2n}\\
                    ... & ... & ... & ...\\
                    \theta_{n1} & \theta_{n2} & ... & \theta_{nn}
                    \end{bmatrix}\\
 ,\mathbf{E}^{exp} = \begin{bmatrix}
                    e_{11} & e_{12} & ... & e_{1n}\\
                    e_{21} & e_{22} & ... & e_{2n}\\
                    ... & ... & ... & ...\\
                    e_{n1} & e_{n2} & ... & e_{nn}
                    \end{bmatrix}\\
  , \mathbf{E}^{log1p} = \begin{bmatrix}
                        l_{11} & l_{12} & ... & l_{1n}\\
                        l_{21} & l_{22} & ... & l_{2n}\\
                        ... & ... & ... & ...\\
                        l_{n1} & l_{n2} & ... & l_{nn}
                        \end{bmatrix}\\
\end{displaymath}

In \textbf{Sinusoid}-embedding, we convert each $d_{ij}$ into a vector $\theta_{ij} \in \mathbb{R}^{h}$, by applying the following transformation:
\begin{displaymath}
  \theta_{ij, 2k} = sin(\frac{d_{ij}}{freq^{\frac{2k}{h}}})\\
  , \theta_{ij, 2k+1} = cos(\frac{d_{ij}}{freq^{\frac{2k}{h}}})
\end{displaymath}
where $\theta_{ij, k}$ is the $k^{th}$ value of the vector $\theta_{ij}$ and $freq$ is an adjustable parameter.

For \textbf{Exp} and \textbf{Log1p} embeddings, we apply the following transformations:
\begin{displaymath}
  e_{ij, k} = exp(\frac{-|d_{ij}|}{freq^{\frac{k}{h}}})\\
  , l_{ij, k} = log(1 + \frac{|d_{ij}|}{freq^{\frac{k}{h}}})
\end{displaymath}

Each embedding offers a distinctive view on time intervals. For example, larger gaps between time will quickly decay to zero in $\mathbf{E}^{exp}$, while in $\mathbf{E}^{log1p}$ they will slowly increase to a value that is still manageable in neural networks. These distinctive views enable our self-attention blocks to attend to different parts of the sequence.


Although we intended to explore the vast possibility of encoding functions by devising some of them on our own, we acknowledge that the choice of these functions might seem too improvised. To compensate, we provide a study of a more general form of encoding function with Fourier series in Appendix-\ref{app:fourier}.

==> sections/method_subsections/stacking.tex <==
Given the above definitions, we can create maximum 6 different types of self-attention blocks depending on the type of positional embeddings:
\begin{equation}
    \mathbf{B}_{type}(\mathbf{X}) = \mathbf{B}(\mathbf{X}, \mathbf{E}^{type}) = \mathbf{Z}
\end{equation}

For example, a block of type \textbf{Sinusoid} will compute:
\begin{displaymath}
   \mathbf{B}_{sinusoid}(\mathbf{X}) = \mathbf{B}(\mathbf{X}, \mathbf{E}^{sinusoid}) = \mathbf{Z}
\end{displaymath}

Suppose we decided to use $\Sigma$ different types of self-attention blocks ($\mathbf{B}_{{type}_1}, ..., \mathbf{B}_{{type}_\Sigma}$). We could keep $\Sigma$ blocks on the first layer, and have them take as input the same token embeddings to produce $\Sigma$ outputs: 
\begin{equation}
    [\mathbf{B}^1_{{type}_1}, ..., \mathbf{B}^1_{{type}_\Sigma}](\mathbf{E}^{token}) =
    [\mathbf{B}^1_{{type}_1}(\mathbf{E}^{token}), ..., \mathbf{B}^1_{{type}_\Sigma}(\mathbf{E}^{token})] =
    [\mathbf{Z}^1_1, ..., \mathbf{Z}^1_\Sigma] = \mathbf{Z}^1
\end{equation}
In addition to this, we can stack another $\Sigma$ blocks on the above layer and have them each take the output of the matching block below as input. 
\begin{equation}
    [\mathbf{B}^2_{{type}_1}, ..., \mathbf{B}^2_{{type}_\Sigma}](\mathbf{Z}^1) =
    [\mathbf{B}^2_{{type}_1}(\mathbf{Z}^1_1), ..., \mathbf{B}^2_{{type}_\Sigma}(\mathbf{Z}^1_\Sigma)] =
    [\mathbf{Z}^2_1, ..., \mathbf{Z}^2_\Sigma] = \mathbf{Z}^2
\end{equation}

This process can be repeated to stack a total of $L$ layers, which produce $\mathbf{Z}^L = [\mathbf{Z}^L_1, ..., \mathbf{Z}^L_\Sigma]$ at the end.

Note that the two consecutive blocks (above/below) don't necessarily have to be the same type, but we force them to have the same type. We posited that inconsistent types could hinder the learning process. However, mixing block types could be worthy of future research.

==> sections/method_subsections/token_embedding.tex <==
We keep a learnable embedding matrix $\mathbf{M}^I \in \mathbb{R}^{(|I|+1) \times h}$ for items and a special token \verb|[MASK]|, where $h$ is the dimension of the model. Given $s$, the embedding look-up operation gives us $\mathbf{E}^{token} \in \mathbb{R}^{N \times h}$ :
\begin{displaymath}
  \mathbf{E}^{token} = \begin{bmatrix}
                    m_{s_1}\\
                    m_{s_2}\\
                    ...\\
                    m_{s_n}\\
                    \end{bmatrix}
\end{displaymath}

==> sections/relworks_subsections/self_attention.tex <==
%Recently, a series of Transformer\cite{TRANSFORMER, TRANSFORMER-XL} based models \cite{BERT, XLNET}, which rely purely on multi-headed self-attention mechanism, have provided a strong basis for many tasks in language understanding. They also inspired many self-attention based sequential recommendation models such as SASRec\cite{SASRec} and BERT4Rec\cite{BERT4Rec}.
Given a stack of same-sized vectors, Transformer applies the following scaled dot-product attention:
\begin{displaymath}
  \textrm{Attention}(Q, K, V) = \textrm{softmax}(\frac{QK^T}{\sqrt{d}})V
\end{displaymath}
where $Q, K, V$ are queries, keys, and values each generated by separate linear projections applied to the same input vectors. Multi-headed self-attention differs from single-headed self-attention only in that it creates multiple sets of queries, keys, and values, each producing its own attention results which are concatenated in the final output. The capability of each query to assign more attention to relevant values makes it a powerful mechanism for understanding sequential data.
